Octopus: Enhancing CXL Memory Pods via Sparse Topology

The Compute Express Link (CXL) interconnect enables compute "pods" that pool memory across servers to reduce cost and improve efficiency. These pods also facilitate pairwise communication whose needs conflict with pooling. Importantly, existing pod designs are small or require indirection through expensive switches. These conventional designs implicitly assume that pods must fully connect all servers to all CXL pooling devices. This paper breaks with this conventional wisdom by introducing Octopus pods. Octopus directly connects servers to low-port-count CXL pooling devices (e.g., 4 ports) yet scales to large pods without switches by constructing a sparse CXL topology in which each pooling device connects to a carefully chosen subset of servers. Octopus explicitly balances "overlap", where two servers connect to the same pooling device: overlap reduces pooling efficiency but enables low-latency communication. Octopus resolves this tension by grouping servers into "islands" with low-latency intra-island communication and interconnecting islands to favor pooling. We build a three-server CXL pod prototype and simulate scaled pods with 96 servers under measured device characteristics and physical constraints (1.5 m copper cables). On hardware, Octopus RPCs are 3.2x faster than in-rack RDMA and 2.4x faster than CXL switches. In simulation, Octopus achieves net server cost savings of 3-5.4% whereas CXL switches result in a net cost increase.

==> bg.tex <==
\section{CXL Building Blocks and Existing Designs}\label{sec:existingdesigns}

We review existing multi-ported device (\mpd) and pod designs that motivate our design proposal in Section~\ref{sec:overview}.
Multi-ported CXL \mpds form a key building block for \sysname pods.





\subsection{Existing CXL Pod Designs}\label{sec:excxlpods}

Existing literature proposes either switched CXL pod designs or fully-connected CXL pods based on \mpds.

\subsubsection{Switched CXL Pods}

Any CXL controller (including a single-ported controller) may be connected to a CXL switch, which in turn connects multiple CPUs.
Switched designs resemble tree network topologies in CXL 2.0~\cite{cxl2topology} and Clos network topologies in CXL 3.0~\cite{cxl3fabric}.
A single switch typically offers 128-256 CXL lanes~\cite{xconn2024switch}.
These lanes would be shared among connected CPUs, CXL controllers, and other devices.
For example, 128 lanes could connect six CPUs with x16 CXL ports and two single-ported CXL controllers with x16 ports.
In CXL 3.0, multiple switching levels can be used to build large-scale CXL pods~\cite{das2024introduction}.

The tradeoff for switched designs is higher power, cost, and latency.
Prior work observes that CXL switch costs can exceed the benefits that can be achieved from pooling at scale~\cite{berger2023design,levis2023case}.
CXL switch latency is also fundamentally higher than direct CXL connections, as switches require serialization and deserialization of CXL packets twice on every path from CPU to CXL memory controller~\cite{berger2023design, pond:asplos2023}.
Current switches add more than $250ns$ of latency~\cite{xconn2024latency}, resulting in idle load-to-use latency of roughly $500-600ns$.

From talking with product teams at \azure, we find that these high costs and access latencies exclude switched CXL pods from deployment.

\subsubsection{Fully-connected CXL Pods based on Multi-Headed Devices}

The alternative to switched CXL pods is connecting CPUs directly to \mpds~\cite{pond:asplos2023}.
To our knowledge, all existing proposals assume a fully connected topology where every host/CPU connects to every PD.
%The \mpd port count ($N$) determines how many CPUs are part of the CXL pod.
For example, as shown in Figure~\ref{fig:topexample} five 16-ported \mpds connect to the same 16 CPUs.
Fully-connected topologies have been proposed in official CXL standard presentations by Microchip and Intel~\cite{wagh2021cxl}, and in industry presentations by Seagate~\cite{seagate2024cxl}, ARM~\cite{arm2024cxl}, SK Hynix~\cite{ha2023dynamic}, Microsoft~\cite{pond:asplos2023}, Jackrabbit labs~\cite{mackey2024cxl}, and Unifabrix~\cite{hyatt2023quest}.
The common assumption is that $N$-ported \mpds will create a CXL pod of $N$ CPUs.%\footnote{Some variants assume multiple connections between a single PD and a CPU, using CXL link aggregation.}
In this design, if a CPU is connected to $X$ \mpds, every CPU in the pod connects to the same set of $X$ \mpds.
This ensures that all CPUs can access and allocate memory from any of the $X$ \mpds in the pod.
% This results in a semi-regular bipartite graph, where one part (hosts) has uniform degrees, and the other part (pools) has degrees constrained by N.

Compared to switched topologies, large \mpds reduce cost, power, and latency~\cite{berger2023design}.
However, we find that we can further improve cost and latency \emph{by changing the pod topology}.




